Graphs States and the necessity of Euler Decomposition

Coecke and Duncan recently introduced a categorical formalisation of the interaction of complementary quantum observables. In this paper we use their diagrammatic language to study graph states, a computationally interesting class of quantum states. We give a graphical proof of the fixpoint property of graph states. We then introduce a new equation, for the Euler decomposition of the Hadamard gate, and demonstrate that Van den Nest's theorem--locally equivalent graphs represent the same entanglement--is equivalent to this new axiom. Finally we prove that the Euler decomposition equation is not derivable from the existing axioms.

==> diag/compactg.tex <==
\begin{tikzpicture}[xscale=0.50,yscale=0.50]
\useasboundingbox (-0.5,-0.5) rectangle (2.5,1.5);
\draw (1.00,0.00) -- (0.00,1.00);
\draw (2.00,1.00) -- (1.00,0.00);
\filldraw[fill=green] (1.00,0.00) ellipse (0.20cm and 0.20cm);
\end{tikzpicture}


==> diag/compactr.tex <==
\begin{tikzpicture}[xscale=0.50,yscale=0.50]
\useasboundingbox (-0.5,-0.5) rectangle (2.5,1.5);
\draw (1.00,0.00) -- (0.00,1.00);
\draw (2.00,1.00) -- (1.00,0.00);
\filldraw[fill=red] (1.00,0.00) ellipse (0.20cm and 0.20cm);
\end{tikzpicture}


==> diag/e34.strid.tex <==
matrix{
\\
&&1box4(l3d,r3d,3r3d,5r3d,u)[l,s=ellipse,c=red,w=0.2,h=0.2]&&1box4(3l3d,l3d,r3d,3r3d,u)[l,c=red,w=0.2,h=0.2]&&1box4(5l3d,3l3d,l3d,r3d,u)[l,c=red,w=0.2,h=0.2]&&\\
\\
\\
&0box1(d)[l,c=green,w=0.2,h=0.2]&&0box1(d)[l,c=green,w=0.2,h=0.2]&&0box1(d)[l,c=green,w=0.2,h=0.2]&&0box1(d)[l,c=green,w=0.2,h=0.2]&\\
\\
}


%
%matrix{
%\\
%&mult(u3r,dr,l)[l,w=0.2,h=0.2]&&&&&&mult(u3l,dl,r)&\\
%\\
%&&&&sym(ull,dll,urr,drr)\\
%\\
%&mult(ur,d3r,l)&&&&&&mult(ul,d3l,r)&\\
%\\
%}

==> diag/k22b.tex <==
matrix{
\\
&1box2(l2d,2r4d,u)[l,s=ellipse,c=red,w=0.2,h=0.2]&&1box2(2l4d,r2d,u)[l,c=red,w=0.2,h=0.2]&\\
\\
\\
\\
&1box1(d,l2u)[l,c=green,w=0.2,h=0.2]&&1box1(d,r2u)[l,c=green,w=0.2,h=0.2]&\\
\\
}


%
%matrix{
%\\
%&mult(u3r,dr,l)[l,w=0.2,h=0.2]&&&&&&mult(u3l,dl,r)&\\
%\\
%&&&&sym(ull,dll,urr,drr)\\
%\\
%&mult(ur,d3r,l)&&&&&&mult(ul,d3l,r)&\\
%\\
%}
